Optima: Optimizing Effectiveness and Efficiency for LLM-Based Multi-Agent System

Large Language Model (LLM) based multi-agent systems (MAS) show remarkable potential in collaborative problem-solving, yet they still face critical challenges: low communication efficiency, poor scalability, and a lack of effective parameter-updating optimization methods. We present Optima, a novel framework that addresses these issues by significantly enhancing both communication efficiency and task effectiveness in LLM-based MAS through LLM training. Optima employs an iterative generate, rank, select, and train paradigm with a reward function balancing task performance, token efficiency, and communication readability. We explore various RL algorithms, including Supervised Fine-Tuning, Direct Preference Optimization, and their hybrid approaches, providing insights into their effectiveness-efficiency trade-offs. We integrate Monte Carlo Tree Search-inspired techniques for DPO data generation, treating conversation turns as tree nodes to explore diverse interaction paths. Evaluated on common multi-agent tasks, including information-asymmetric question answering and complex reasoning, Optima shows consistent and substantial improvements over single-agent baselines and vanilla MAS based on Llama 3 8B, achieving up to 2.8x performance gain with less than 10\% tokens on tasks requiring heavy information exchange. Moreover, Optima's efficiency gains open new possibilities for leveraging inference-compute more effectively, leading to improved inference-time scaling laws. By addressing fundamental challenges in LLM-based MAS, Optima shows the potential towards scalable, efficient, and effective MAS (https://chenweize1998.github.io/optima-project-page).

==> sections/analysis.tex <==
\section{Analysis}
\label{sec:analysis}

==> table/main_table_QA.tex <==
\begin{table*}[t]
    \centering
    \caption{The QA main table.}
    \begin{tabular}{l*{10}{c}}
    \toprule
     & \multicolumn{2}{c}{\textbf{Hotpot QA}} & \multicolumn{2}{c}{\textbf{Multi Wiki}} & \multicolumn{2}{c}{\textbf{Trivia QA}} & \multicolumn{2}{c}{\textbf{CBT}}  \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    \textbf{Method} & \textbf{F1} & \textbf{\#Tokens} & \textbf{F1} & \textbf{\#Tokens} & \textbf{F1} & \textbf{\#Tokens} & \textbf{F1} & \textbf{\#Tokens} \\
    % single
    \midrule
    CoT & 0.256 &123.7 &0.205 &139.8 &0.598 &110.3 &0.434&135.3\\
    SC ($n=8$) & 0.338 & 996.3 &0.287 &1052.8 &0.700 &891.4&0.529 &1067.7\\
    % multi
    \midrule
    MAD &  0.284 & 570.9 &0.259&543.7 & 0.710 & 408.6 & 0.538 & 493.0\\
    AutoForm & 0.282 & 97.7 &0.247 & 117.7 & 0.609 & 74.0 & 0.350 &64.8\\
    % train
    \midrule
    ISFT & \underline{0.545} & 67.6  & \underline{0.724} & 61.2 & \underline{0.719} & \underline{51.5} & \textbf{0.718} & \underline{38.5}\\
    IDPO & 0.525 & \underline{45.7} &0.661&\textbf{35.9} &0.693 & 69.2 & 0.667 & \textbf{37.2}\\
    ISFT-DPO &  \textbf{0.600} & \textbf{29.5} & \textbf{0.742} & \underline{54.9} & \textbf{0.771} & \textbf{32.5} & \underline{0.701} & 38.9\\
    \midrule
    Multi SC & 0 & 0& 0.770 &1023.8 & 0 & 0 & 0 & 0 \\
    \bottomrule
    \end{tabular}
    \label{tab:qa-main-table}
    \vspace{-1 em}
\end{table*}


==> table/main_table_debate.tex <==
\begin{table*}[t]
    \centering
    \caption{The debate main table.}
    \begin{tabular}{l*{6}{c}}
    \toprule
     & \multicolumn{2}{c}{\textbf{MATH}} & \multicolumn{2}{c}{\textbf{GSM8k}} & \multicolumn{2}{c}{\textbf{ARC Challenge}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
    \textbf{Method} & \textbf{Accuracy} & \textbf{\#Tokens} & \textbf{Accuracy} & \textbf{\#Tokens} & \textbf{Accuracy} & \textbf{\#Tokens}\\
    % single
    \midrule
    CoT & 0.238 & 378.8 & 0.627 &213.9 & 0.652 &138.9\\
    SC ($n=8$) & 0.353 & 3170.0 & 0.742 & 1105.8 &0.756 & 1116.7\\
    % multi
    \midrule
    MAD & 0.213 & 1123.5 & 0.725 & 514.7 & 0.714 &478.0\\
    AutoForm & 0.269 & 641.3& 0.710 &410.5 & 0.602 & 221.2\\
    % train
    \midrule
    ISFT & 0 & 0& 0.784& 286.0& 0.761 & 100.2\\
    IDPO & 0 & 0 & 0.785 & 270.1& 0.745 & 97.8\\
    ISFT-DPO &0 & 0 & 0&0 & 0.760 & 118.1 \\
    \midrule
    Multi SC & \\
    \bottomrule
    \end{tabular}
    \label{tab:debate-main-table}
    \vspace{-1 em}
\end{table*}

